Layer-Dependent Importance Sampling for Training Deep and Large Graph Convolutional Networks

Graph convolutional networks (GCNs) have recently received wide attentions, due to their successful applications in different graph tasks and different domains. Training GCNs for a large graph, however, is still a challenge. Original full-batch GCN training requires calculating the representation of all the nodes in the graph per GCN layer, which brings in high computation and memory costs. To alleviate this issue, several sampling-based methods have been proposed to train GCNs on a subset of nodes. Among them, the node-wise neighbor-sampling method recursively samples a fixed number of neighbor nodes, and thus its computation cost suffers from exponential growing neighbor size; while the layer-wise importance-sampling method discards the neighbor-dependent constraints, and thus the nodes sampled across layer suffer from sparse connection problem. To deal with the above two problems, we propose a new effective sampling algorithm called LAyer-Dependent ImportancE Sampling (LADIES). Based on the sampled nodes in the upper layer, LADIES selects their neighborhood nodes, constructs a bipartite subgraph and computes the importance probability accordingly. Then, it samples a fixed number of nodes by the calculated probability, and recursively conducts such procedure per layer to construct the whole computation graph. We prove theoretically and experimentally, that our proposed sampling algorithm outperforms the previous sampling methods in terms of both time and memory costs. Furthermore, LADIES is shown to have better generalization accuracy than original full-batch GCN, due to its stochastic nature.

==> section/our-method.tex <==
We present our method in this section. As illustrated in the aforementioned sections, when performing large-scale training of GCN, the size of receptive fields dramatically. Therefore, node sampling methods are applied to construct the forward computation graph of GCN, which further leads to approximate gradient evaluations. However, there are some shortcomings in existing sampling methods. For node-wise sampling methods including GraphSAGE \citep{graphsage} and VR-GCN \citep{DBLP:conf/icml/ChenZS18}, one has to sample a certain number of nodes in the neighbor set of all sampled nodes in the current layer. Apparently, the number of nodes that are selected to build the computation graph is exponentially large with the number of hidden layers. Regarding layer-wise sampling that samples the required nodes at the beginning of each iteration in each layer, then builds the computation graph based on the sampled nodes to update the model weights. However, the existing layer-wise sampling scheme \citep{DBLP:journals/corr/abs-1801-10247} is not efficient when the graph is sparse, since some nodes may have no neighbor been sampled during the sampling process, which results in unmeaningful zero activations \citep{DBLP:conf/icml/ChenZS18}.

To address the aforementioned drawbacks and weakness of the existing sampling methods for GCN training, we propose our sampling algorithms that can efficiently take advantage of nodes as well as reduce sampling complexity. In specific, we organize our sampling method as three parts: sampling set characterization; importance sampling scheme; variance-reduced estimator.



\subsection{Layer-wise Importance sampling }
Previously we have illustrate our sampling idea, i.e., the sampling set at the $l-1$-th layer is determined by the nodes we have sampled at the $l$-th layer. Assuming at the $l$-th layer we sample $n_l = |\cS_l|$ nodes (at the last layer we uniformly take $n_L$ nodes from training set for batch training), the output of GCN (embeddings at the last layer) can be formulated in the following way:
\begin{align*}
\tilde\Zb_{L} = \tilde\Pb^{(L-1)}\tilde \Hb^{(L-1)}\Wb^{(L-1)}
\end{align*}
where $\tilde \Pb^{(L-1)}\in \RR^{n_L\times n_{L-1}}$ denotes the modified Laplacian matrix after sampling and $\tilde \Hb^{(l-1)}\in \RR^{n_{L-1}\times d_{l-1}}$ denotes the approximated activations of nodes in the set $\cS_{l-1}$. similarly, at each layer, we have $\tilde\Zb_l = \tilde\Pb^{(l-1)}\tilde \Hb^{(L-1)}\Wb^{(l-1)}$.
Note that this procedure can be described as matrix multiplication with sketching. Let $\Sbb_l\in\RR^{n\times n_{l}}$ and $\Sbb_{l-1}\RR^{n\times n_{l-1}}$ be the sketching matrices at the $l$-th layer and $l-1$-th layer respectively, we have $\Zb_l = \Sbb_l^\top\Pb\Sbb_{l-1}\Sbb_{l-1}^\top \tilde \Hb^{(l-1)}\Wb^{(l-1)}$. 
Note that at the $l$-th layer, we need to sample $n_l$ nodes from the set $\cV_l$. Then for each sample $\xi$, we assign non-uniform probability $p_i = Pr(\xi = i)\ge 0$ with $\sum_{i\in\cV_l}p_i = 1$.
Then let $\{i_k^{(l)}\}_{k\in\cS_l}$ be the indices of nodes in $\cS_l$ and assume $i_1^{(l)}\le i_2^{(l)}\dots\le i_{n_l}^{(l)}$, the the sketching matrix $\Sbb_l$ is defined as follows
\begin{align*}
\Sbb_l(i,j) = \left\{
 \begin{array}{ll}
        \frac{1}{\sqrt{p_i^{(l)}}},& (i,j) = (i_{k}^{(l)}, k);\\
        0,& otherwise.
    \end{array}
\right.
\end{align*}
Specifically, at the last layer we set $p_i^{L} = 1/n_L$ for all $i\in \cS_L$.
Now, we are able to rewrite the output of GCN as follows,
\begin{align*}
\tilde \Zb_L & = \Sbb_L^\top\Pb\Sbb_{L-1}\Sbb_{L-1}^\top \tilde \Hb^{(L-1)}\Wb^{(L-1)}\notag\\
& = \Sbb_L^\top\Pb\Sbb_{L-1}\Sbb_{L-1}^\top  \sigma\big(\Pb\Sbb_{L-2}\Sbb_{L-2}^\top\tilde \Hb^{(L-2)}\Wb^{(L-2)}\big)\Wb^{(L-2)}\notag\\
& = \Sbb_L^\top\Pb\Sbb_{L-1}\Sbb_{L-1}^\top  \sigma\big(\Pb\Sbb_{L-2}\Sbb_{L-2}^\top \cdots \sigma\big(\Pb\Sbb_{0}\Sbb_{0}^\top\Xb\Wb_0\big)\cdots\Wb^{(L-2)}\big)\Wb^{(L-2)}.
\end{align*}
Then there raises a question, which sampling scheme is the optimal to achieve smallest error in terms of the output $\tilde \Zb_l$. Following \cite{DBLP:journals/corr/abs-1801-10247}, we are going to exploit important sampling method to alleviate the variance of the proposed estimator. Since we adopt upper-down strategy to build the computation graph, we cannot access the activations of nodes in the previous layer to help design the distribution of important sampling in the current layer. Therefore, the construction of important distribution only depends on the sampling results in the upper layers. 
%Based on this, we provide two important sampling methods: approximate important sampling and layer-wise important sampling.

Our goal is to minimize the mean square error (MSE) $\EE[\|\tilde\Zb_L - \Zb_L\|_F^2]$, where $\Zb_L= \Sbb_L^\top \Pb \Hb^{(L-1)}\Wb^{(L-1)}$ is the exact output of GCN for nodes in the current training batch. Note that
\begin{align*}
\Zb_L - \tilde\Zb_L  &= \Sbb_L^\top\Pb\Hb^{(L-1)}\Wb^{(L-1)} -\Sbb_L^\top \Pb \Sbb_{L-1}\Sbb_{L-1}^\top\tilde \Hb^{(l-1)}\Wb^{(L-1)} \notag\\
& = \Sbb_L^\top \Pb(\Ib - \Sbb_{L-1}\Sbb_{L-1}^\top)\Hb^{(L-1)}\Wb^{(L-1)} + \Sbb_L^\top \Pb \Sbb_{L-1}\Sbb_{L-1}^\top\big(\Hb^{(L-1)} - \tilde\Hb^{(L-1)}\big)\Wb^{(L-1)}.
\end{align*}
Moreover, for each $l\le L-1$, we have
\begin{align}\label{eq:diff_activation}
\Hb^{(l-1)} - \tilde \Hb^{(l-1)} &= \sigma\big(\Pb \Hb^{(l-2)}\Wb^{(l-2)}\big)- \sigma\big(\Pb\Sbb_{l-2}\Sbb_{l-2}^\top\tilde \Hb^{(l-2)}\Wb^{(l-2)}\big) \notag\\
& =  \sigma\big(\Pb \Hb^{(l-2)}\Wb^{(l-2)}\big)-\sigma\big(\Pb \Sbb_{l-2}\Sbb_{l-2}^\top\Hb^{(l-2)}\Wb^{(l-1)}\big) \notag\\
&\quad + \sigma\big(\Pb \Sbb_{l-2}\Sbb_{l-2}^\top\Hb^{(l-2)}\Wb^{(l-2)}\big) -\sigma\big(\Pb\Sbb_{l-2}\Sbb_{l-2}^\top\tilde \Hb^{(l-2)}\Wb^{(l-2)}\big).
\end{align}
Then we propose the following two sampling mechanisms.
% \subsubsection{Sampling mechanism I}
% Since we only focus on the variance introduced by sampling, and note that activation function is $1$-Lipschitz, therefore we replace the activation function $\sigma(\cdot)$ with linear model, which yields
% \begin{align*}
% \Hb^{(L-1)} - \tilde \Hb^{(L-1)}&\simeq \Pb (\Ib - \Sbb_{L-2}\Sbb_{L-2}^\top) \Hb^{(L-2)}\Wb^{(L-2)} + \Pb \Sbb_{L-2}\Sbb_{L-2}^\top\big(\Hb^{(L-2)}-\tilde\Hb^{(L-2)}\big)\Wb^{(L-2)}.
% \end{align*}
% Recursively applying the above approximation, we obtain
% \begin{align*}
% \EE[\|\Zb_L - \tilde \Zb_L\|_F^2] &\simeq \EE\bigg[ \bigg\|\Sbb_L^\top\sum_{l=0}^{L-1}\bigg( \bigg(\prod_{s = L-1}^{l+1}\Pb\Sbb_{s}\Sbb_{s}^\top\bigg)\Pb(\Ib - \Sbb_{l}\Sbb_{l}^\top)\Hb^{(l)}\bigg(\prod_{s = l}^{L-1}\Wb^{(s)}\bigg)\bigg)\bigg\|_F^2\bigg]\notag\\
% &\le L \sum_{l=0}^{L-1}\EE\bigg[\bigg\|\Sbb_L^\top\bigg( \bigg(\prod_{s = L-1}^{l+1}\Pb\Sbb_{s}\Sbb_{s}^\top\bigg)\Pb(\Ib - \Sbb_{l}\Sbb_{l}^\top)\Hb^{(l)}\bigg(\prod_{s = l}^{L-1}\Wb^{(s)}\bigg)\bigg)\bigg\|_F^2\bigg]\notag\\
% &: = L\sum_{l=0}^{L-1}\EE\big[\big\|\tilde\Ub_l(\Ib-\Sbb_l\Sbb_l^\top)\Vb_l\|_F^2\big],
% \end{align*}
% where $\tilde\Ub_l$ is random but $\Vb_l$ is fixed.
% Let $\cV_{l}$ be the union of neighbors of  nodes we sampled in the $l+1$-th layer, and let $\tilde \Lb_{l}$ be a $n\times n$ diagonal matrix with $\tilde \Lb_{l}(i,i) = 1$ if $v_i\in \cV_l$ and $\tilde \Lb_{l}(i,i) = 0$ otherwise. We have $\tilde\Ub_l\Vb_l = \tilde\Ub_l\tilde \Lb_l\Vb_l$. Since the sampling scheme of $\Sbb_l$ is determined with fixed $\{\Sbb_s\}_{s>l}$, therefore we can set the probability for all nodes as 
% \begin{align*}
% p_i^{(l)} = \frac{\|\tilde\Ub_l(:,i)\|_2^2}{\|\tilde\Ub_l\|_F^2}.
% \end{align*}
% Evidently, the probability of nodes which are not included in the set $\cV_l$ is zero since there is no nonzero entry in the corresponding columns of $\Ub_l$. Therefore, the update formula for the $i$-th activation in the $l+1$-th layer can be expressed as
% \begin{align*}
% \tilde h^{(l+1)}_i = \sigma\bigg(\sum_{j\in\cS_l}\frac{\Pb(i,j)\tilde h^{(l)}_j\Wb^{(l)}}{p_i^{(l)}n_l}\bigg), \quad j\sim \{p_i^{(l)}\}_{i\in \cV_l}, \quad l=0,1,\dots,L-1.
% \end{align*}
% Note that we only required to compute activations $\tilde h_i^{(l+1)}$ for all $i\in\cS_{l+1}$. 
% % Note that this estimation is much more precise than that in \cite{DBLP:journals/corr/abs-1801-10247} (see (10) in their paper) since a) we characterize a much smaller feasible set for sampling which could avoid invalid samples and b) our important probability mass function can aggregate the information
% Moreover, based on such importance sampling mechanism, we have 
% \begin{align*}
% \EE\big[\big\|\tilde\Ub_l(1-\Sbb_l\Sbb_l^\top)\Vb_l\|_F^2\big] &=\EE\big[\EE\big[\big\|\Ub_l(1-\Sbb_l\Sbb_l^\top)\Vb_l\|_F^2|\tilde\Ub_l\big] \big]\notag\\
% &=\frac{1}{n_l}\EE\big[\|\tilde\Ub_l\|_F\|\tilde \Lb_l\Vb_l\|_F^2 - \| \tilde\Ub_l\Vb_l\|_F^2 \big] .
% \end{align*}
% Applying the above equality for all $l$, we obtain
% \begin{align*}
% \EE[\|\Zb_L - \tilde \Zb_L\|_F^2] &\simeq\EE\bigg[ \bigg\|\sum_{l=0}^{L-1}\tilde \Ub_l(\Ib - \Sbb_l\Sbb_l^\top)\Vb^{(l)}\bigg\|_F^2\bigg]\notag\\
% &\le L\sum_{l=0}^{L-1}\frac{1}{n_l}\EE\big[\|\tilde\Ub_l\|_F\|\tilde \Lb_l\Vb_l\|_F^2 - \| \tilde\Ub_l\Vb_l\|_F^2 \big].
% \end{align*}
\subsubsection{Sampling mechanism II}
This sampling mechanism starts from \eqref{eq:diff_activation}. Rather than replacing the activation function with linear model, we direct optimize the difference $\tilde\Hb^{l} - \Hb^{l}$ layer by layer. 
%Note that 
% \begin{align*}
% &\Hb^{(l)} - \tilde \Hb^{(l)} \notag\\
% & =  \sigma\big(\Pb \Hb^{(l-1)}\Wb^{(l-1)}\big)-\sigma\big(\Pb \Sbb_{l-1}\Sbb_{l-1}^\top\Hb^{(l-1)}\Wb^{(l)}\big) \notag\\
% &\quad + \sigma\big(\Pb \Sbb_{l-1}\Sbb_{l-1}^\top\Hb^{(l-1)}\Wb^{(l-1)}\big) -\sigma\big(\Pb\Sbb_{l-1}\Sbb_{l-1}^\top\tilde \Hb^{(l-1)}\Wb^{(l-1)}\big)\notag\\
% &=  \sigma\big(\Pb \Hb^{(l-1)}\Wb^{(l-1)}\big)-\sigma\big(\Pb \Sbb_{l-1}\Sbb_{l-1}^\top\Hb^{(l-1)}\Wb^{(l)}\big) \notag\\
% &\quad + \sigma\big(\Pb \Sbb_{l-1}\Sbb_{l-1}^\top\sigma(\Pb\Hb^{(l-2)}\Wb^{(l-2)})\Wb^{(l-1)}\big) -\sigma\big(\Pb\Sbb_{l-1}\Sbb_{l-1}^\top \sigma(\Pb\Sbb_{l-2}\Sbb_{l-2}^\top\Hb^{(l-2)}\Wb^{(l-2)})\Wb^{(l-1)}\big)\notag\\
% &+\sigma\big(\Pb \Hb^{(l-1)}\Wb^{(l-1)}\big)-\sigma\big(\Pb \Sbb_{l-1}\Sbb_{l-1}^\top\Hb^{(l-1)}\Wb^{(l)}\big) \notag\\
% &\quad + \sigma\big(\Pb \Sbb_{l-1}\Sbb_{l-1}^\top\sigma(\Pb\Sbb_{l-2}\Sbb_{l-2}^\top\Hb^{(l-2)}\Wb^{(l-2)})\Wb^{(l-1)}\big) -\sigma\big(\Pb\Sbb_{l-1}\Sbb_{l-1}^\top \sigma(\Pb\Sbb_{l-2}\Sbb_{l-2}^\top\tilde\Hb^{(l-2)}\Wb^{(l-2)})\Wb^{(l-1)}\big)\notag\notag\\
% =
% \end{align*}
Let $f_l(\Xb) = \sigma(\Pb\Xb^{(l)}\Wb^{(l)})$ and $\tilde f_l(\Xb) = \sigma(\Pb\Sbb_l\Sbb_l^\top\Xb\Wb^{(l)})$, we can expand $\Hb^{(L)} - \tilde\Hb^{(L)}$ as
\begin{align*}
\Hb^{(L)} - \tilde\Hb^{(L)}&= f_{L-1}(\Hb^{(L-1)}) - \tilde f_{L-1}(\Hb^{(L-1)}) + \tilde f_{L-1}(\Hb^{(L-1)}) - \tilde f_{L-1}(\tilde\Hb^{(L-1)})\notag\\
&=f_{L-1}(\Hb^{(L-1)}) - \tilde f_{L-1}(\Hb^{(L-1)}) + \tilde f_{L-1}\circ f_{L-2}(\Hb^{L-2}) - \tilde f_{L-1}\circ \tilde f_{L-2}(\Hb^{L-2}) \notag\\
&\quad+ \tilde f_{L-1}\circ \tilde f_{L-2}(\Hb^{(L-2)}) -\tilde f_{L-1}\circ \tilde f_{L-2}(\tilde\Hb^{(L-2)}) \notag\\
& = \sum_{l=0}^{L-1}\big[\tilde f_{L-1}\circ\tilde f_{L-2}\circ\cdots\circ  f_{l}(\Hb^{(l)})-\tilde f_{L-1}\circ\tilde f_{L-2}\circ\cdots\circ \tilde f_{l}(\Hb^{(l)})\big].
\end{align*}
Then we focus on each element in the above summation. Note that
\begin{align}\label{eq:var_scheme2}
&\big\|\tilde f_{L-1}\circ\tilde f_{L-2}\circ\cdots\circ  f_{l}(\Hb^{(l)})-\tilde f_{L-1}\circ\tilde f_{L-2}\circ\cdots\circ \tilde f_{l}(\Hb^{(l)})\big\|_F\notag\\
&\le \|\Pb\Sbb_{L-1}\Sbb_{L-1}^\top\|_2\|\Wb^{(L-1)}\|_2\|\tilde f_{L-2}\circ\cdots\circ  f_{l}(\Hb^{(l)})-\tilde f_{L-2}\circ\cdots\circ \tilde f_{l}(\Hb^{(l)})\|_F\notag\\
& \le \bigg(\prod_{s = l+2}^{L-1}\|\Pb\Sbb_{l}\Sbb_{l}^\top\|_2\|\Wb^{(l)}\|_2\bigg)\|\tilde f_{l+1}\circ f_l(\Hb^{(l)}) - \tilde f_{l+1}\circ\tilde f_l(\Hb^{(l)})\|_F.
\end{align}
Moreover, we have
\begin{align*}
&\tilde f_{l+1}\circ f_l(\Hb^{(l)}) - \tilde f_{l+1}\circ\tilde f_l(\Hb^{(l)}) \notag\\
&= \sigma\big(\Pb\Sbb_{l+1}\Sbb_{l+1}^\top \sigma(\Pb\Hb^{(l)})\Wb^{(l+1)}\big) - \sigma\big(\Pb\Sbb_{l+1}\Sbb_{l+1}^\top \sigma(\Pb\Sbb_{l}\Sbb_{l}^\top\Hb^{(l)})\Wb^{(l+1)}\big)\notag\\
&=\sigma\big(\Pb\Sbb_{l+1}\Sbb_{l+1}^\top \sigma(\tilde\Qb_{l+1}\Pb\Hb^{(l)}\Wb^{(l)})\Wb^{(l+1)}\big) - \sigma\big(\Pb\Sbb_{l+1}\Sbb_{l+1}^\top \sigma(\tilde\Qb_{l+1}\Pb\Sbb_{l}\Sbb_{l}^\top\Hb^{(l)}\Wb^{(l)})\Wb^{(l+1)}\big),
\end{align*}
% \begin{align*}
% \Sbb_{l}\Sbb_{l}^\top(\Hb^{l} - \tilde\Hb^l) &= \Sbb_{l}\Sbb_{l}^\top\tilde\Lb_l(\Hb^{l} - \tilde\Hb^l)\notag\\
% &=\Sbb_{l}\Sbb_{l}^\top\big[\sigma\big(\tilde\Lb_l\Pb \Hb^{(l-1)}\Wb^{(l-1)}\big)-\sigma\big(\tilde\Lb_l\Pb \Sbb_{l-1}\Sbb_{l-1}^\top\Hb^{(l-1)}\Wb^{(l)}\big)\big] \notag\\
% &\quad + \Sbb_{l}\Sbb_{l}^\top\big[\sigma\big(\Pb \Sbb_{l-1}\Sbb_{l-1}^\top\Hb^{(l-1)}\Wb^{(l-1)}\big) -\sigma\big(\Pb\Sbb_{l-1}\Sbb_{l-1}^\top\tilde \Hb^{(l-1)}\Wb^{(l-2)}\big)\big],
% \end{align*}
where $\tilde \Lb_l$ is a diagonal matrix such that $\tilde \Lb_l(i,i) = 1$ if $v_i\in\cV_i$ and $\tilde \Lb_l(i,i) = 0$ otherwise. Then, we have the following upper bound regarding the norm $\|\tilde f_{l+1}\circ f_l(\Hb^{(l)}) - \tilde f_{l+1}\circ\tilde f_l(\Hb^{(l)})\|_F$
\begin{align*}
\|\tilde f_{l+1}\circ f_l(\Hb^{(l)}) - \tilde f_{l+1}\circ\tilde f_l(\Hb^{(l)})\|_F\le \|\Pb\Sbb_{l+1}\Sbb_{l+1}^\top\|_2\|\Wb^{(l+1)}\|_2\|\tilde\Qb_{l+1}\Pb\Hb^{(l)}\Wb^{(l)} - \tilde\Qb_{l+1}\Pb\Sbb_{l}\Sbb_{l}^\top\Hb^{(l)}\Wb^{(l)}\|_F.
\end{align*}
The rest step is to apply important sampling to optimize the norm $\|\tilde\Qb_{l+1}\Pb\Hb^{(l)}\Wb^{(l)} - \tilde\Qb_{l+1}\Pb\Sbb_{l}\Sbb_{l}^\top\Hb^{(l)}\Wb^{(l)}\|_F$. Note that given all $\Sbb_{s}$ with $s\ge l+1$, we have $\EE\big[\tilde\Qb_{l+1}\Pb\Hb^{(l)}\Wb^{(l)} - \tilde\Qb_{l+1}\Pb\Sbb_{l}\Sbb_{l}^\top\Hb^{(l)}\Wb^{(l)}\big]= 0$. Then we can assign the following probabilities to all nodes
\begin{align*}
 p_i^{(l)} = \frac{\|\tilde \Ub_l(:,i)\|_2^2}{\|\tilde \Ub_l\|_F^2},   
\end{align*}
where $\tilde \Ub_l = \tilde \Qb_{l+1}\Pb$. Therefore, given all $\Sbb_s$ with $s\ge l+1$, we have
\begin{align}\label{eq:var_onelayer}
\EE\big[\big\|\tilde\Qb_{l+1}\Pb\Hb^{(l)}\Wb^{(l)} - \tilde\Qb_{l+1}\Pb\Sbb_{l}\Sbb_{l}^\top\Hb^{(l)}\Wb^{(l)}\big\|_F^2\big] &= \frac{1}{n_l}\big(\|\tilde \Qb_{l+1}\Pb \|_F^2\|\tilde\Lb_{l}\Hb^{(l)}\Wb^{(l)}\|_F^2 - \|\tilde\Qb_{l+1}\Pb\Hb^{(l)}\Wb^{(l)}\|_F^2\big)\notag\\
&\le \frac{1}{n_l}\|\tilde \Qb_{l+1}\Pb \|_F^2\|\tilde\Lb_{l}\Hb^{(l)}\Wb^{(l)}\|_F^2,
\end{align}
where the last inequality holds due to $\Sbb_l$ is randomly generated from the set $\cV_l$ rather than $[n]$. 
Plugging this back into \eqref{eq:var_scheme2}, we have
\begin{align*}
&\EE\big[\big\|\tilde f_{L-1}\circ\tilde f_{L-2}\circ\cdots\circ  f_{l}(\Hb^{(l)})-\tilde f_{L-1}\circ\tilde f_{L-2}\circ\cdots\circ \tilde f_{l}(\Hb^{(l)})\big\|_F^2\big]\notag\\
&\le \frac{1}{n_l}\EE\bigg[\bigg(\prod_{s = l+1}^{L-1}\|\Pb\Sbb_{l}\Sbb_{l}^\top\|_2^2\|\Wb^{(l)}\|_2^2\bigg)\|\tilde\Qb_{l+1}\Pb\|_F^2\|\tilde\Lb_l\Hb^{(l)}\Wb^{(l)}\|_F^2\bigg].
\end{align*}
\subsection{Comparison with existing sampling methods}
Since all existing sampling methods for training GCN only consider single-layer variance, we only compare our variance results of sampling mechanism for one particular layer with existing ones. Assume at $l+1$-th layer, we have to approximate a set of nodes, denoted by $\cS_{l+1}$, via aggregating the activations of sampled nodes at the $l$-th layer. In this part we compare our method with Naive neighbor sampling and FastGCN. As shown in \eqref{eq:var_onelayer}, let $\tilde\Zb^{(l+1)} = \Pb\Sbb_l\Sbb_l^\top\Hb^{(l)}\Wb^{(l)}$ be the embeddings of nodes in the $l+1$-th layer, 
the variance of our sampling method for all nodes in $\cS_{l+1}$ can be formulated as
\begin{align*}
\text{var}(\tilde\Qb_{l+1}\tilde \Zb^{(l+1)}) &= \frac{1}{n_l}\big(\|\tilde \Qb_{l+1}\Pb \|_F^2\|\tilde\Lb_{l}\Hb^{(l)}\Wb^{(l)}\|_F^2 - \|\tilde\Qb_{l+1}\Pb\Hb^{(l)}\Wb^{(l)}\|_F^2\big)\notag\\
& = \frac{1}{n_l}\bigg(\sum_{i\in\cS_{l+1}}D_i\sum_{i\in\cV_{l}}\|\hb_i^{(l)}\Wb^{(l)}\|_2^2- \sum_{i\in\cS_{l+1}}\bigg\|\zb_i^{(l+1)}\bigg\|_2^2\bigg).
\end{align*}
where $D_i$ is the degree of $v_i$.
Then we are going to present the variance of neighbor sampling. Assume for node $v_i$ in $\cS_{l+1}$ we sample $m_i$ neighbors in the set $\cN(v_i)$, therefore the total variance can be calculated as
\begin{align*}
\text{var}(\tilde\Qb_{l+1}\tilde \Zb^{l+1}) = \sum_{i\in\cS_{l+1}}\text{var}(\tilde\zb^{(l+1)}_i). 
\end{align*}
Note that
\begin{align*}
\text{var}(\tilde\zb^{(l+1)}_i) = \frac{1}{m_i}\bigg(|\cN(v_i)|\sum_{j\in\cN(v_i)}\|h_j^{(l)}\Wb^{(l)}\|_2^2 - \|\zb_i^{(l+1)}\|_2^2\bigg),
\end{align*}
which leads to the following variance of $\tilde\Qb_{l+1}\tilde \Zb^{(l+1)}$,
\begin{align*}
\sum_{i\in\cS_{l+1}}\frac{|\cN(v_i)|}{m_i}\sum_{j\in\cN(v_i)}\|h_j^{(l)}\Wb^{(l)}\|_2^2  - \sum_{i\in\cS_{l+1}}\frac{\|\zb_i^{(l+1)}\|_2^2}{m_i}.
\end{align*}
 Then assume the norm $\|\hb_i^{(l)}\Wb^{(l)}\|_2^2$ is in the constant order for all $i$, then the variance of our method is in the order of $O(|\cS_{l+1}|\bar D|\cV_l|/n_l)$, while the variance of NS is $O(|\cS_{l+1}|\bar D^2/m)$, where $\bar D$ and $m$ is the average degree and neighbor samples.
Since in our sampling method $\cV_l = \cup_{i\in\cS_{l+1}}\cN(v_i)$, therefore we have $|\cV_l|\le \sum_{i\in\cS_{l+1}}|\cN(V_i)| = O(|\cS_{l+1}|\bar D)$.
This further implies using the same number of samples, i.e., $n_l = O(|\cS_{l+1}|m)$, the variance of our method is in the order of $O(|\cV_l|\bar D/m)$, which is smaller than that of NS, i.e., $O(|\cS_{l+1}|\bar D^2/m)$. This improvement can be much more significant if the graph is not that sparse, i.e., many neighbors are shared.

Then we derive the variance of FastGCN, where the important sampling procedure is performed in the same way for all layers. Specifically, the probabilities assigned to nodes are
\begin{align*}
p_i = \frac{\|\Pb(:, i)\|_2^2}{\|\Pb\|_F^2}.    
\end{align*}
Assuming we sample $n_l$ nodes, it can be directly computed that the variance of $\tilde\Qb_{l+1}\tilde \Zb^{(l+1)}$ is
\begin{align*}
\text{var}(\tilde\Qb_{l+1}\tilde \Zb^{(l+1)}) &= \frac{1}{n_l}\bigg(\|\Pb\|_F^2\sum_{i=1}^n\frac{\|\tilde \Qb_{l+1}\Pb(:,i)\|_2^2\|\Hb^{(l)}\Wb^{(l)}(i,:)\|_2^2}{\|\Pb(:,i)\|_2^2} -\|\tilde\Qb_{l+1}\Pb\Hb^{(l)}\Wb^{(l)}\|_F^2 \bigg)\notag\\
&=O(\bar D|\cS_{l+1}|n/n_l),
\end{align*}
where assume that $\|\hb_i^{(l)}\Wb^{(l)}\|_2^2$ is bounded by some constant for all $i$. Evidently, the variance of FastGCN is much worse than our method since the total number of node $n$ is much larger than $|\cV_l|$ when the graph is large or the batch size is small.
 
